SPECTRE: An FFT-Based Efficient Drop-In Replacement to Self-Attention for Long Contexts

Long-context transformers face significant efficiency challenges due to the quadratic cost of self-attention. However, many modern applications-from multi-turn dialogue to high-resolution vision-require contexts spanning tens of thousands of tokens. We introduce SPECTRE, a method that replaces each attention head with a fast real FFT, a content-adaptive spectral gate, and an inverse FFT, reducing per-layer complexity from $\mathcal{O}(L^{2})$ to $O(L\log L)$ while preserving the surrounding architecture. We extend this efficiency to autoregressive generation through our Prefix-FFT cache and enhance local feature representation with an optional wavelet module that adds negligible computational overhead. Our experiments demonstrate that SPECTRE operates up to 7$\times$ faster than FlashAttention-2 on 128k-token contexts while matching or exceeding baseline performance on PG-19 language modeling and ImageNet-1k classification tasks. SPECTRE achieves these improvements by adding fewer than 6\% parameters to the base model, making hundred-kilotoken context processing feasible on commodity GPUs without specialized hardware.

==> plots/plot2.tex <==
% % ------------------------------------------------------------------
% % Prefix–FFT Cache (Pre-fill + Decode) — standalone figure
% % ------------------------------------------------------------------
% \documentclass[tikz,border=6pt]{standalone}

% % --- fonts ---------------------------------------------------------
% \usepackage{newtxtext,newtxmath}
% \usepackage[scaled=0.85]{inconsolata}
% \renewcommand{\ttdefault}{zi4}
% \usepackage{amsmath}

% % --- TikZ setup ----------------------------------------------------
% \usepackage[x11names,table]{xcolor}
% \usepackage{tikz}
% \usetikzlibrary{positioning,fit,calc,arrows.meta,
%   shadows.blur,backgrounds,
%   shapes.geometric,shapes.symbols}

% \pgfdeclarelayer{bg}
% \pgfsetlayers{bg,main}

% % --- colours -------------------------------------------------------
% \definecolor{OpBlue}     {HTML}{4472C4}
% \definecolor{DataOrange} {HTML}{E69138}
% \definecolor{FFTGreen}   {HTML}{009E73}
% \definecolor{GatePurple} {HTML}{7E2F8E}
% \definecolor{PhaseGrey}  {gray}{0.25}

% % ---- common dimensions -------------------------------------------
% \newlength\RectW   \setlength\RectW{3cm}   % final outside width
% \newlength\ShapeW  \setlength\ShapeW{2.4cm}% inner text width for shaped nodes

% % ---- node / arrow styles -----------------------------------------
% \tikzset{
%   arr/.style={-{Stealth[length=2mm,width=1.6mm]},thick},
%   phasebox/.style={draw=PhaseGrey,dashed,thick,
%                    rounded corners=4pt,inner sep=4pt},
%   % plain rectangles ------------------------------------------------
%   op/.style={
%     draw=OpBlue!70,fill=OpBlue!10,thick,rounded corners=3pt,
%     blur shadow={shadow xshift=0.7pt,shadow yshift=-0.7pt},
%     text width=\RectW,minimum height=1.05cm,
%     align=center,font=\footnotesize,inner sep=3pt,outer sep=0pt},
%   datarect/.style={
%     draw=DataOrange!70,fill=DataOrange!10,thick,rounded corners=3pt,
%     blur shadow={shadow xshift=0.7pt,shadow yshift=-0.7pt},
%     text width=\RectW,minimum height=1.05cm,
%     align=center,font=\footnotesize,inner sep=3pt,outer sep=0pt},
%   % special shapes --------------------------------------------------
%   dataset/.style={
%     draw=DataOrange!70,fill=DataOrange!10,thick,
%     shape=cylinder,shape border rotate=90,aspect=0.18,
%     text width=\ShapeW,minimum width=\RectW,
%     align=center,font=\footnotesize,inner sep=3pt,outer sep=0pt},
%   fft/.style={
%     draw=FFTGreen!70,fill=FFTGreen!10,thick,
%     shape=trapezium,trapezium angle=60,aspect=0.1,
%     transform shape,            % <-- scales the whole node (text included)
%     scale=0.45,                 % <-- was 0.7; lower = smaller
%     shape border uses incircle,
%     text width=\ShapeW,minimum width=\RectW,
%     align=center,font=\Large,inner sep=3pt,outer sep=0pt},
%   gate/.style={
%     draw=GatePurple!70,fill=GatePurple!10,thick,
%     shape=regular polygon,regular polygon sides=6,
%     shape border rotate=90,shape border uses incircle,
%     transform shape,            % <-- add this
%     scale=0.45,                 % <-- new (no scale before)
%     text width=\ShapeW,minimum width=\RectW,
%     align=center,font=\Large,inner sep=3pt,outer sep=0pt},
% }

% % ------------------------------------------------------------------
% \begin{document}
% \begin{tikzpicture}[node distance = 1.2cm and 2.4cm]

% % ---------- PRE-FILL (left column) ---------------------------------
% \node[op]           (prompt)    {Prompt\\$V,Q$ ($L\!\le\!N_{\max}$)};
% \node[op, below=of prompt]      (pad) {Zero-pad to $N_{\max}$};
% \node[fft, below=of pad]        (fft) {$\mathcal{R}_{N_{\max}}$\\Real FFT};
% \node[dataset, below=of fft]    (prefixfft)
%     {\texttt{prefix\_fft}\\$(\tfrac{N_{\max}}{2}\!+\!1)\!\times\!d$};

% \node[dataset, right=2.6cm of pad] (ring)
%     {Ring buffers\\\texttt{V\_buf}, \texttt{Q\_buf}\\$N_{\max}\!\times\! d$};

% \node[datarect, below=1.3cm of ring] (sumq) {Running sum\\$\texttt{sum\_q}$};

% % internal arrows
% \draw[arr] (prompt) -- (pad);
% \draw[arr] (pad)    -- (fft);
% \draw[arr] (fft)    -- (prefixfft);
% \draw[arr] (pad.east) ++(0.1,0) -- ++(0.9,0) |- (ring.west);
% \draw[arr] (ring) -- (sumq);

% % dashed frame + label
% \node[phasebox, fit=(prompt)(prefixfft)(ring)(sumq)] (prefbox) {};
% \node[anchor=south west,font=\bfseries\large,text=PhaseGrey]
%       at (prefbox.north west) {Pre-fill (one-shot)};
% \node[anchor=north west,font=\scriptsize,align=left]
%       at ($(prefixfft.south west)+(0pt,-4pt)$)
%       {$\mathcal{O}\!\bigl(N_{\max}\log N_{\max}\,d\bigr)$\\{\it one time}};

% % ---------- DECODE (right column) ----------------------------------
% \node[op,   right=7cm of prompt] (newtok) {Incoming\\token $v_t,q_t$};
% \node[op,   below=of newtok]     (evict)  {(a) Evict \&\\Update FFT};
% \node[op,   below=of evict]      (refresh){(b) Refresh buffers\\\& $\texttt{sum\_q}$};
% \node[gate, below=of refresh]    (gate)   {(c) Spectral gate\\MLP $\Rightarrow g$};
% \node[gate, below=of gate]       (phase)  {(d) Inject positional\\phase};
% \node[fft,  below=of phase]      (ifft)   {(e) Inverse FFT\\$\widetilde{V}$};

% % decode arrows
% \draw[arr] (newtok) -- (evict);
% \draw[arr] (evict)  -- (refresh);
% \draw[arr] (refresh)-- (gate);
% \draw[arr] (gate)   -- (phase);
% \draw[arr] (phase)  -- (ifft);

% % cross-phase arrows ------------------------------------------------
% \draw[arr] (ring.east) to[out= 10,in=170,looseness=1.1]  (evict.west);
% \draw[arr] (ring.east) to[out=-10,in=170,looseness=1.15] (refresh.west);

% \begin{pgfonlayer}{bg}      % deep sweep behind everything
%   \draw[arr] (prefixfft.east)
%              to[out=-10,in=185,looseness=1.35] (evict.west);
% \end{pgfonlayer}

% \draw[arr] (prefixfft.east) to[out=-15,in=185,looseness=1.2] (ifft.west);
% \draw[arr] (sumq.east)      to[out= 10,in=180,looseness=1.05] (gate.west);

% % dashed frame + label
% \node[phasebox, fit=(newtok)(ifft)] (decbox) {};
% \node[anchor=south west,font=\bfseries\large,text=PhaseGrey]
%       at (decbox.north west) {Decode (per-token)};
% \node[anchor=north west,font=\scriptsize]
%       at ($(ifft.south west)+(0pt,-4pt)$)
%       {$\mathcal{O}\!\bigl(\tfrac{N_{\max}}{2}d\bigr)$ per step};

% \end{tikzpicture}
% \end{document}

